Testing Partially-Identifiable Causal Queries Using Ternary Tests

We consider hypothesis testing of binary causal queries using observational data. Since the mapping of causal models to the observational distribution that they induce is not one-to-one, in general, causal queries are often only partially identifiable. When binary statistical tests are used for testing partially-identifiable causal queries, their results do not translate in a straightforward manner to the causal hypothesis testing problem. We propose using ternary (three-outcome) statistical tests to test partially-identifiable causal queries. We establish testability requirements that ternary tests must satisfy in terms of uniform consistency and present equivalent topological conditions on the hypotheses. To leverage the existing toolbox of binary tests, we prove that obtaining ternary tests by combining binary tests is complete. Finally, we demonstrate how topological conditions serve as a guide to construct ternary tests for two concrete causal hypothesis testing problems, namely testing the instrumental variable (IV) inequalities and comparing treatment efficacy.

==> ci.tex <==
\section{Conditional Independence}\label{sec:CI}
Mediation graph (without confounding, like the Berkeley case) - similar to XOR case, Collider detection in an unshielded triple like \citet{GuoRichardson20}? 

Can expand the null like in the fairness paper with the constraint that the induced set of observational distributions remains constant. Interesting things happen for example, if $\distq \cup \distqalt \neq \Delta$, expanding the null can make the space of unidentifiable models shrink. Cook up an example.

==> three-arm-testing.tex <==
\section{Ternary Testing}\label{sec:three-arm}
In this section, we present a few straightforward extensions of the standard binary null hypothesis testing framework to a ternary hypothesis testing framework; a case that often occurs while developing statistical tests for causal hypotheses and in causal discovery \citep{RobinsSSW03} \citep{ZhangSpirtes08}. 

\begin{table}\centering\setlength\tabcolsep{3.5pt}\renewcommand\arraystretch{1.25}

  \makebox[\textwidth]{%
    \begin{tabular}{|l|*{3}{c|}}
      \hline
      \diagbox[width=\dimexpr \textwidth/6+2\tabcolsep\relax, height=1.2cm]{Outcome}{Truth}
        & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
      \hline
      $0$ & True Negative & \textbf{False} Negative & \textbf{False} Confidence \\
      \hline
      $1$ & \textbf{False} Positive & True Positive & \textbf{False} Confidence \\
      \hline
      $\idk$ &Doubt & Doubt & True Doubt \\
      \hline
    \end{tabular}
  }
   \caption{Outcome-Truth table for ternary hypothesis testing. The cells that include \textbf{False} are considered errors. This scenario considers the case where being conservative in the decision is not penalized.}
 \label{tab:truth}
\end{table}

Consider two sets of distributions where $\nll$ is the null hypothesis and $\alt$ is the alternative hypothesis. Table~\ref{tab:truth_all_error} summarizes a outcome-truth table for ternary hypothesis testing. As in binary hypothesis testing, we consider false positives and false negatives to be errors. Although we define a ternary hypothesis testing setup that deems an error to be whenever the decision is contrary to the truth, we note that in our case the interpretation of the intersection $\nll \cap \alt$ allows relaxations of the notions of error. We refer to a `test' $\test$ as a sequence of tests $\Paren{\phi_1, \phi_2, \cdots, \phi_n, \cdots}$ where the subscript denotes the sample-size. When the sample-size is unspecified, we will abuse notation to refer to the outcome of a test, $\test$, given a sample $X$, by $\test\Paren{X}$. 

%Since we consider the intersection $\nll \cap \alt$ to be parameters where the truth is unidentifiable, we deem providing a definitive decision in such a case an error While we consider deciding $\idk$ to be an error if the truth is unambiguous, i.e., $\nll \setminus \alt$ or $\alt \setminus \nll$, one could relax that while considering ``non-trivial'' tests where the notion of non-triviality is such that asymptotically a test decides unambiguously. 

The critical region of a test in the binary hypothesis testing setup is defined by a single set in the space of observations. In a ternary hypothesis testing setup, we denote the partitions of the observation space where the test concludes definitively as the ``critical regions''. Specifically, we define a test as a tuple $(K_0, K_1)$ where $K_0 = \left \{ x \in \mathcal{X} : \test(x) = 0 \right \}$, $K_1 = \left \{ x \in \mathcal{X} : \test(x) = 1 \right \}$, and the set of observations belonging to $\cX \setminus \Paren{K_0 \cup K_1}$ is where the test outputs $\idk$.

The size and power of a binary hypothesis test, whose critical region is $K$, is specified by the power function $\pi\Paren{P; K}: P \mapsto P\Paren{X \in K}$ where the size of the test is given by $\sup\limits_{P \in \nll} \pi(P;K)$. A straightforward extension for a ternary hypothesis test is a pair of functions $\Paren{\pi\Paren{P; K_0},\pi\Paren{P; K_1}}$ where $\pi\Paren{P; K_0} : P \mapsto P\Paren{X \in K_0}$ and $\pi\Paren{P; K_1} : P \mapsto P\Paren{X \in K_1}$. The motivation for the size of a test in a binary frequentist hypothesis testing framework is an upper bound on the probability of a Type I error or false-positive error rate since the stakes to reject the null hypothesis, given the alternative hypothesis is true, are assumed to be higher. However this is not necessarily the case in the ternary hypothesis testing setup. Therefore, we define the size of a ternary hypothesis test to be a tuple of values one for each error in Table~\ref{tab:truth_all_error} 
%$$\Paren{\sup\limits_{\theta \in \nll\setminus \alt} \pi(\theta;K_1),\sup\limits_{\theta \in \alt\setminus\nll} \pi(\theta;K_0),\sup\limits_{\theta \in \nll \cap \alt} \pi(\theta;K_0) + \pi(\theta;K_1)}.$$
%\todo{in the definition of size, the last value can also be max of the two.}

\subsection{Ternary Testing by Combining Binary Tests}

A natural way to obtain ternary tests is by combining two or more binary tests. In general, overlapping hypotheses $\nll$ and $\alt$ partition $\nll \cup \alt$ in three disjoint partitions, $\nll \setminus \alt, \alt \setminus \nll$ and $\nll \cap \alt$. Therefore, we consider a sequence of binary tests that first tests for one of these three partitions and then based on the outcome of this first test, tests for the other two. In this section, we relate the properties of the resulting ternary tests in terms of the properties of its constituent binary tests. 

Consider two binary tests $\test_{1}, \test_{2}$ where the former tests the null hypothesis $\nll \cap \alt$ against its complement in $\nll \cup \alt$, and the latter tests the null hypothesis $\nll \setminus \alt$ against the alternative $\alt \setminus \nll$. The combined ternary test is defined as 
\begin{equation}\label{eq:test_inter_disj}
 \test(x) = 
    \begin{cases}
     \idk & \text{ if } \test_{1}(x)=0, \\
     0 & \text{ if } \test_{1}(x)=1, \test_{2}(x)=0, \\
    1 & \text{ if } \test_{1}(x)=1, \test_{2}(x)=1.
    \end{cases}
\end{equation}
Denote the false positive and false negative error rates for the constituent binary tests, $\test_{1}$ and $\test_{2}$ by $\fone_{1}, \fzero_{1}$, and $\fone_{2}, \fzero_{2}$, respectively. We will now list the error rate bounds for each of the $6$ errors in Table~\ref{tab:truth_all_error}. A summary for this particular definition of $\test_1, \test_2$ is in Table~\ref{tab:error_inter}.

\textbf{0-False-D and 1-False-D}: The error rates for these errors are given by 
\begin{align*}
    &\sup\limits_{\param \in \nll \setminus \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=\idk} = \sup\limits_{\param \in \nll \setminus \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{1,n}\Paren{X^n}=0},\\
    &\sup\limits_{\param \in \alt \setminus \nll} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=\idk} = \sup\limits_{\param \in \alt \setminus \nll} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{1,n}\Paren{X^n}=0}
\end{align*}
respectively. Since 
\begin{equation*}
    \sup\limits_{\param \in \Paren{\alt \setminus \nll} \cup \Paren{\nll \setminus \alt}} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{1,n}\Paren{X^n}=0} \leq \fzero_1,  
\end{equation*}
\begin{equation*}
    \max\Paren{\sup\limits_{\param \in \nll \setminus \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=\idk},\sup\limits_{\param \in \alt \setminus \nll} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=\idk}} \leq \fzero_1. 
\end{equation*}

\textbf{False-0 and False-1}: The error rates for these errors are given by 
\begin{align*}
    \sup\limits_{\param \in \alt \setminus \nll} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=0} &= \sup\limits_{\param \in \alt \setminus \nll} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{1,n}\Paren{X^n}=1 \cap \test_{2,n}\Paren{X^n}=0 }\\
    &\leq \sup\limits_{\param \in \alt \setminus \nll} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{2,n}\Paren{X^n}=0} \leq \fzero_2,
\end{align*}
\begin{align*}
    \sup\limits_{\param \in \nll \setminus \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=1} &= \sup\limits_{\param \in \nll \setminus \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{1,n}\Paren{X^n}=1 \cap \test_{2,n}\Paren{X^n}=1} \\
    &\leq \sup\limits_{\param \in \nll \setminus \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{ \test_{2,n}\Paren{X^n}=1} \leq \fone_2
\end{align*}
respectively. 

\textbf{False-c-0 and False-c-1}: The error rates are given by
\begin{align*}
    &\sup\limits_{\param \in \nll \cap \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=0} &= \sup\limits_{\param \in \nll \cap \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{1,n}\Paren{X^n}=1 \cap \test_{2,n}\Paren{X^n}=0 }\\
    &\sup\limits_{\param \in \nll \cap \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_n\Paren{X^n}=1} &= \sup\limits_{\param \in \nll \cap \alt} \limsup\limits_{n \rightarrow \infty} \param^n\Paren{\test_{1,n}\Paren{X^n}=1 \cap \test_{2,n}\Paren{X^n}=1} 
\end{align*}
respectively. 
Since 
\begin{align*}    &\param^n\Paren{\test_{1,n}\Paren{X^n}=1 \cap \test_{2,n}\Paren{X^n}=1} + \param^n\Paren{\test_{1,n}\Paren{X^n}=1 \cap \test_{2,n}\Paren{X^n}=0 }\\
&=\param^n\Paren{\test_{1,n}\Paren{X^n}=1},
\end{align*}
we can bound both the error rates by $\fone_1$.

A similar analysis holds for the case where $\test_1$ first tests $\nll \setminus \alt$ versus $\alt$ and then $\test_2$ tests $\nll \cap \alt$ versus $\alt \setminus \nll$, and for the case where $\test_1$ first tests $\alt \setminus \nll$ versus $\nll$ and then $\test_2$ tests $\nll \cap \alt$ versus $\nll \setminus \alt$. We summarize the error rates for the ternary tests obtained by combining various sequences of binary tests in Table~\ref{tab:global}.

% \begin{table}\centering\setlength\tabcolsep{3.5pt}\renewcommand\arraystretch{1.25}
%  \makebox[\textwidth]{%
% \begin{tabular}{|l|*{3}{c|}}
%       \hline
%       \diagbox[width=\dimexpr \textwidth/5+2\tabcolsep\relax, height=1.2cm]{\makecell[c]{\hspace{0.7em}\vspace{0.2em}{\rotatebox{0}{Decision}}}}{\makecell[c]{\vspace{-0.8em}{\rotatebox{0}{Truth}}}}
%         & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
%       \hline
%       $0$ & True $0$ & \textbf{False} $0$ & \textbf{False}-C-$0$ \\
%       \hline
%       $1$ & \textbf{False} $1$ & True $1$ & \textbf{False}-C-$1$ \\
%       \hline
%       $\idk$ &0-\textbf{False}-D & 1-\textbf{False}-D & True Doubt \\
%       \hline
%     \end{tabular}
% }   \caption{Decision-Truth table for ternary hypothesis testing. The cells that include \textbf{False} are considered errors.}\label{tab:truth_all_error}
% \end{table}

\begin{table}
\caption{}\label{tab:global}
    \begin{subtable}[t]{0.45\textwidth}
\begin{tabular}{|l|*{3}{c|}}
      \hline
      \diagbox[width=\dimexpr \textwidth/5+2\tabcolsep\relax, height=1.2cm]{\makecell[c]{\hspace{0em}\vspace{0.1em}{\rotatebox{327}{\footnotesize{Decision}}}}}{\makecell[c]{\vspace{-0.8em}{\rotatebox{327}{\footnotesize{Truth}}}}}
        & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
      \hline
      $0$ & True $0$ & \textbf{False} $0$ & \textbf{False}-C-$0$ \\
      \hline
      $1$ & \textbf{False} $1$ & True $1$ & \textbf{False}-C-$1$ \\
      \hline
      $\idk$ &0-\textbf{False}-D & 1-\textbf{False}-D & True Doubt \\
      \hline
    \end{tabular}
         \caption{Decision-Truth table for a general ternary test. All off-diagonal cells are considered errors.}\label{tab:truth_all_error}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.45\textwidth}
    \begin{tabular}{|l|*{3}{c|}}
      \hline
      \diagbox[width=\dimexpr \textwidth/5+2\tabcolsep\relax, height=1.2cm]{\makecell[c]{\hspace{0.2em}{\rotatebox{327}{\footnotesize{Decision}}}}}{\makecell[c]{{\rotatebox{324}{\footnotesize{Truth}}}}}
        & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
      \hline
      $0$ & - & $\fzero_2$ & $\fone_1$ \\
      \hline
      $1$ & $\fone_2$ & - & $\fone_1$\\
      \hline
      $\idk$ & $\fzero_1$ & $\fzero_1$ & - \\
      \hline
    \end{tabular}
    \caption{$\test = \Paren{\test_{1},\test_{2}}$ where $\test_1: \nll \cap \alt \text{ vs } (\nll \cap \alt)^\complement$, $\test_2: \nll \setminus \alt \text{ vs } (\alt \setminus \nll)$.} \label{tab:error_inter}
    \end{subtable}

    \begin{subtable}[t]{0.45\textwidth}
    \begin{tabular}{|l|*{3}{c|}}
      \hline
      \diagbox[width=\dimexpr \textwidth/5+2\tabcolsep\relax, height=1.2cm]{\makecell[c]{\hspace{0.2em}{\rotatebox{327}{\footnotesize{Decision}}}}}{\makecell[c]{{\rotatebox{324}{\footnotesize{Truth}}}}}
        & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
      \hline
      $0$ & - & $\fzero_1$ & $\fzero_1$ \\
      \hline
      $1$ & $\fone_1$ & - & $\fone_2$\\
      \hline
      $\idk$ & $\fone_1$ & $\fzero_2$ & - \\
      \hline
    \end{tabular}
    \caption{$\test = \Paren{\test_{1},\test_{2}}$ where $\test_1: \nll \setminus \alt \text{ vs } \alt$, $\test_2: \nll \cap \alt \text{ vs } (\alt \setminus \nll)$.} \label{tab:error_0}
    \end{subtable}\hfill
    \begin{subtable}[t]{0.45\textwidth}
    \begin{tabular}{|l|*{3}{c|}}
      \hline
      \diagbox[width=\dimexpr \textwidth/5+2\tabcolsep\relax, height=1.2cm]{\makecell[c]{\hspace{0.2em}{\rotatebox{327}{\footnotesize{Decision}}}}}{\makecell[c]{{\rotatebox{324}{\footnotesize{Truth}}}}}
        & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
      \hline
      $0$ & - & $\fone_1$ & $\fone_2$ \\
      \hline
      $1$ & $\fzero_1$ & - & $\fzero_1$\\
      \hline
      $\idk$ & $\fzero_2$ & $\fone_1$ & - \\
      \hline
    \end{tabular}
    \caption{$\test = \Paren{\test_{1},\test_{2}}$ where $\test_1: \alt \setminus \nll \text{ vs } \nll$, $\test_2: \nll \cap \alt \text{ vs } (\nll \setminus \alt)$.} \label{tab:error_1}
    \end{subtable}
    \begin{subtable}[t]{0.45\textwidth}
    \begin{tabular}{|l|*{3}{c|}}
      \hline
      \diagbox[width=\dimexpr \textwidth/5+2\tabcolsep\relax, height=1.2cm]{\makecell[c]{\hspace{0.2em}{\rotatebox{327}{\footnotesize{Decision}}}}}{\makecell[c]{{\rotatebox{324}{\footnotesize{Truth}}}}}
        & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
     \hline
      $0$ & - & $\fzero_1$ & $\fzero_2$ \\
      \hline
      $1$ & $\fone_1$ & - & $\fone_1$\\
      \hline
      $\idk$ & $\fone_2$ & $\fzero_1$ & - \\
      \hline
    \end{tabular}
    \caption{$\test = \Paren{\test_{1},\test_{2}}$ where $\test_1: \nll \text{ vs } \alt\setminus \nll$, $\test_2: (\nll \setminus \alt) \text{ vs } \nll \cap \alt$.} \label{tab:error_1_rej_1}
    \end{subtable}\hfill
    \begin{subtable}[t]{0.45\textwidth}
    \begin{tabular}{|l|*{3}{c|}}
      \hline
      \diagbox[width=\dimexpr \textwidth/5+2\tabcolsep\relax, height=1.2cm]{\makecell[c]{\hspace{0.2em}{\rotatebox{327}{\footnotesize{Decision}}}}}{\makecell[c]{{\rotatebox{324}{\footnotesize{Truth}}}}}
        & $\nll \setminus \alt$ & $\alt  \setminus \nll$ & $\nll \cap \alt$ \\
      \hline
      $0$ & - & $\fzero_1$ & $\fone_2$ \\
      \hline
      $1$ & $\fone_1$ & - & $\fone_1$\\
      \hline
      $\idk$ & $\fzero_2$ & $\fzero_1$ & - \\
      \hline
    \end{tabular}
    \caption{$\test = \Paren{\test_{1},\test_{2}}$ where $\test_1: \nll \text{ vs } \alt \setminus \nll$, $\test_2: \nll \cap \alt \text{ vs } (\nll \setminus \alt)$.} \label{tab:error_1_rej_setminus}
    \end{subtable}
\end{table}

\subsubsection{Existence of Tests based on Topological Conditions}

So far we assumed the existence of binary tests $\test_1$ and $\test_2$ with certain false positive and false negative rates. Topological properties of the null and alternative hypothesis characterize the existence of binary tests that satisfy certain desiderata in terms of consistency and error rate control \citep{DemboPeres94, GeninKelly17, Kleijn22, BoekenSGM25}. \todo{Fill this with details}

In this section we take as starting point the assertion that if a null hypothesis $\nll_*$ with a disjoint alternative hypothesis $\alt_*$ is closed in the weak topology on $\nll_* \uplus \alt_*$, then for all $\fone \in (0,1)$, there exists a binary test $\test$ such that a) its false positive error rate is controlled asymptotically, i.e., 
\begin{equation*}
    \sup\limits_{P \in \nll_*} \limsup\limits_{n \rightarrow \infty} P^n\Paren{\test_n(X^n)=1} \leq \fone,
\end{equation*}
and b) the test is pointwise consistent under the alternative, i.e., 
\begin{equation*}
     \liminf\limits_{n \rightarrow \infty} P^n\Paren{\test_n(X^n)=1} =1
\end{equation*}
for all $P \in \alt_*$. \todo{Adjust the notion of false-one error control based on Philip's results for clopen hypothesis sets?} Further, if $\nll_*$ is clopen in the weak topology on $\nll_* \uplus \alt_*$ (implying that $\alt_*$ is also clopen in the weak topology on $\nll_* \uplus \alt_*$), then in addition to properties (a) and (b) above, we get asymptotic false negative error control as well, i.e., for all $\fone \in (0,1)$ and $\fzero \in (0,1)$, there exists a binary test $\test$ such that (a) and (b) hold, and, c) the test's false negative error is controlled asymptotically, i.e., 
\begin{equation*}
    \sup\limits_{P \in \alt_*} \limsup\limits_{n \rightarrow \infty} P^n\Paren{\test_n(X^n)=0} \leq \fzero.
\end{equation*}

Consider a \textit{two-stage} ternary hypothesis testing setup where we first test a pair of disjoint hypotheses in $\nll \cup \alt$, denoted by $(\nll_1, (\nll_1)^\complement))$ such that either $\nll_1$ or $(\nll_1)^\complement$ is one of the three disjoint sets $\nll\setminus \alt, \nll \cap \alt$ or $\alt \setminus \nll$ (which implies that the complement is the disjoint union of the remaining two). If the result of the first binary test results in concluding in favor of one of the three disjoint partitions, we terminate the test. Otherwise, the binary test concludes in favor of the union of two of the disjoint partitions, and therefore, we continue with binary testing of the remaining two disjoint partitions. Note that the above description of combining two binary tests contains many possible choices of combinations. Given the topological constraints on hypotheses, not all combinations are testable in the first place. However, we show that for arbitrary $\nll, \alt$, we can find a combination such that the first pair of hypotheses is testable and even more surprisingly, for such a case, for the second-stage, there exists a choice of hypotheses where both the null and alternative hypotheses are clopen, implying asymptotic error control for both error rates. 

\begin{theorem}\label{thm:combine-binary}
For arbitrary $\nll$ and $\alt$, there always exists a sequence of pairs of disjoint hypothesis sets $\Paren{\nll_{first},(\nll_{first})^\complement}$ and $\Paren{\nll_{second},\alt_{second}}$ such that a) $\nll_{first}$ is closed, b) either $\nll_{first}$ is one of the three disjoint $\nll\setminus \alt, \nll \cap \alt$ or $\alt \setminus \nll$, and $\nll_{second} \uplus \alt_{second} = (\nll_{first})^\complement$ or $(\nll_{first})^\complement$ is one of the three disjoint $\nll\setminus \alt, \nll \cap \alt$ or $\alt \setminus \nll$, and $\nll_{second} \uplus \alt_{second} = \nll_{first}$, and c) both $\nll_{second}$ and $\alt_{second}$ are clopen.
\end{theorem}

\begin{proof}
For arbitrary $\nll, \alt$, consider the three disjoint partitions $\nll \setminus \alt, \nll \cap \alt$ and $\alt \setminus \nll$. Since we cannot have that all are closed or all are open in the weak topology on $\nll \cup \alt$, we either have a) two of these sets are closed and the other is open, or b) two of these sets are open and the other is closed. 

For a) denote the sets as $S_{c_1}$, $S_{c_2}$ and $S_o$. Then the hypotheses $(S_o^\complement, S_o)$ are such that the null is closed in the weak topology on $\nll \cup \alt$, and the alternative is open in the same weak topology. For the second-stage, note that $S_{c_1} \cup S_{c_2} = S_o^\complement$ and consider the hypotheses $(S_{c_1},S_{c_2})$. In the weak topology on $\Paren{\nll \cup \alt} \setminus S_o$, the set $S_{c_1}$ and $S_{c_2}$ are still closed because of the fact that the weak topology on $\Paren{\nll \cup \alt} \setminus S_o$ is a subspace topology of the weak topology on $\nll \cup \alt$. However, since $S_{c_1}$ and $S_{c_2}$ are complements of each other in $\Paren{\nll \cup \alt} \setminus S_o$, they are open, and therefore they are clopen. 

For b) denote the sets as $S_{o_1}$, $S_{o_2}$ and $S_c$. Then the hypotheses $(S_c,S_c^\complement)$ are such that the null is closed in the weak topology on $\nll \cup \alt$, and the alternative is open in the same weak topology. For the second-stage, note that $S_{o_1} \cup S_{o_2} = S_c^\complement$ and consider the hypotheses $(S_{o_1},S_{o_2})$. In the weak topology on $\Paren{\nll \cup \alt} \setminus S_c$, the set $S_{o_1}$ and $S_{o_2}$ are still open because of the fact that the weak topology on $\Paren{\nll \cup \alt} \setminus S_c$ is a subspace topology of the weak topology on $\nll \cup \alt$. However, since $S_{o_1}$ and $S_{o_2}$ are complements of each other in $\Paren{\nll \cup \alt} \setminus S_c$, they are closed, and therefore they are clopen. 

\end{proof}

% The implication of Theorem~\ref{thm:combine-binary} for the properties of the resulting ternary test are interesting. 

% \subsection{Brute-force}

% Consider the test in \eqref{eq:test_inter_disj}. We consider the properties of $\test$ as a function of whether each of the binary tests $\test_{1}$ and $\test_{2}$ achieve Type-I error control, Type-II error control or asymptotic consistency defined as follows. 

% \begin{definition}
% A test $\test$ achieves uniform Type-I error control of $\fone \in \Paren{0,1}$ if for all $\theta \in \nll, \Pr_{\theta}\Paren{\test_n(X_n)=1} \leq \fone$ for all $n$. 
% \end{definition}
% \begin{definition}
% A test $\test$ achieves asymptotic Type-I error control of $\fone \in \Paren{0,1}$ if for all $\theta \in \nll$, $$\limsup\limits_{n \rightarrow \infty} \Pr_{\theta}\Paren{\test_n(X_n)=1} \leq \fone.$$
% \end{definition}
% \begin{definition}
% A test $\test$ achieves uniform Type-II error control of $\fzero \in \Paren{0,1}$ if for all $\theta \in \alt, \Pr_{\theta}\Paren{\test_n(X_n)=0} \leq \fzero$ for all $n$. 
% \end{definition}

% \begin{definition}
% A test $\test$ achieves asymptotic Type-II error control of $\fzero \in \Paren{0,1}$ if for all $\theta \in \alt$, $$\limsup\limits_{n \rightarrow \infty} \Pr_{\theta}\Paren{\test_n(X_n)=0} \leq \fzero.$$
% \end{definition}

% \begin{definition}
% A test $\test$ achieves asymptotic consistency if for all $i$, for all $\theta \in H^{i}$, $$\Pr_{\theta}\Paren{\test_n(X_n)=i} \rightarrow 1.$$ 
% \end{definition}



==> unobs.tex <==
\section{Unobserved Variables} 
Even when we observe all variables, identifiability issues arise if we don't assume faithfulness or positivity. Given that these assumptions are often made implicitly, unidentifiable queries then arise solely as a consequence of not observing all variables. In the aforementioned setup, we can view this as a two-stage process illustrated in Figure~\ref{fig:hyporelations_unobs}. \todo{Expand and define terms.}

Consider causal models defined on variables $\enop \cup \exrv$ where $\exrv$ are hidden exogenous variables with atleast two children in the causal graph and $\enop$ are observed variables \todo{make more precise}. We define $\nullcausaldistqhidden \triangleq \left \{ \model \in \MM: P_{\model, \exrv} \in \distqhiddenall \right \}$ where $\distqhiddenall$ is defined as the set of joint distributions over $\enop, \exrv$ induced by models in $\nullcausalq$. The alternative $\altcausaldistqhidden$ is defined as the complement of $\nullcausaldistqhidden$ in $\MM$. Finally, we define $\nullcausaldistq \triangleq \left \{ \model \in \MM : P_{\model} \in \distq \right \}$ where $\distq$ is now the set of distributions obtained as marginals of $\distqhiddenall$. We denote this mapping that defines the marginal as $\phi_{mg}$. 

The above definitions help us disentangle two sources of unidentifiability, namely the one arising from the mapping of models to unobserved joint distributions, and the one arising from the marginalization. To illustrate each of these in a simple example, we consider the case from Section~\ref{sec:xor}, but while allowing for confounding. Note that this example was also studied in \citet{RobinsSSW03}.

\begin{figure}[t]
     \centering
            \begin{tikzpicture}
            \tikzstyle{vertex}=[circle,fill=none,draw=black,minimum size=17pt,inner sep=0pt]
%\node[vertex] (S) at (0,0) {$S$};
%\node[vertex] (A) at (2,0) {$A$};
%\node[vertex] (D) at (1,1) {$D$};
% \node[align=center] (model) at (0,2.3) {Causal \\ Model \\ Space};
% \node[align=center] (dist) at (4,2.3) {Unobserved \\ Distribution \\ Space};
% \node[align=center] (dist) at (8,2.3) {Observed \\ Distribution\\ Space};
\node (H^0_Q) at (0,1) {$\nullcausalq$};
\node (H^1_Q) at (0,0) {$\altcausalq$};
\node (below) at (0,-0.6) {($\altcausaldistqhidden \cup \altnonid$)};
\node (H^0_{PQH}) at (4,1) {$\nullcausaldistqhidden$};
\node (H^1_{PQH}) at (4,0) {$\altcausaldistqhidden$};
\node (below) at (4,-0.6) {($\altcausaldistq \cup \altdistqhiddennonid$)};
\node (H^0_{PQ}) at (8,1) {$\nullcausaldistq$};
\node (H^1_{PQ}) at (8,0) {$\altcausaldistq$};
\path (H^0_Q) edge node [above]{$\gamma_{all}^{-1} \circ \gamma_{all}$} (H^0_{PQH});
\path (H^1_Q) edge (H^0_{PQH});
\path (H^1_Q) edge (H^1_{PQH});
\path (H^0_{PQH}) edge node [above]{$\gamma_{mg}^{-1} \circ \gamma_{mg}$}  (H^0_{PQ});
\path (H^1_{PQH}) edge (H^1_{PQ});
\path (H^1_{PQH}) edge (H^0_{PQ});

            \end{tikzpicture}
        \caption{Statistical testing of a causal query $Q$ where some variables are hidden. $\gamma_{all}$ maps causal models to unobserved distributions and $\gamma_{mg} = \phi_{mg} \circ \gamma_{all}$ where $\phi_{mg}$ maps unobserved distributions to observed distributions by marginalizing unobserved variables. Note that since composing two surjective functions is surjective, $\gamma_{mg}$ is also surjective.}
        \label{fig:hyporelations_unobs}
\end{figure}


==> xor.tex <==
\section{XOR case}\label{sec:xor}
\begin{figure}[t]
     \centering
            \begin{tikzpicture}
            \tikzstyle{vertex}=[circle,fill=none,draw=black,minimum size=17pt,inner sep=0pt]
\node[vertex] (X) at (0,0) {$X$};
\node[vertex] (Y) at (2,0) {$Y$};
\path (X) edge[red] (Y);
\end{tikzpicture}
\caption{Causal graph for $\model \in \modelfamxor$.} 
\label{fig:xor}
\end{figure}

Consider a family of SCMs, $\modelfamxor$, where $\enop = \left \lbrace X,Y \right \rbrace$ with $|\cX| = |\cY| = 2$, $\exrv = \left \lbrace U_X,U_Y \right \rbrace$, the causal mechanisms are $f_X(U_X) = U_X, f_Y(X,U_Y)$, and the exogenous distribution, $P$, over the independent binary exogenous random variables is a product Bernoulli distribution where $U_X \sim \text{Ber}(p_0), U_Y \sim \text{Ber}(p_1)$. The exogenous distribution induces an observational distribution over the endogenous variables $X,Y$ denoted by $P_{\model}$. For models in $\modelfamxor$, Figure~\ref{fig:xor} illustrates a causal graph of models where $X$ is a parent of $Y$ which we denote by $G$. Note that $\modelfamxor$ also contains models where the causal graph does not include the edge $X \rightarrow Y$. 

%The set of unfaithful observational distributions w.r.t. $G$ is denoted by $U(G)$ and is the set of distributions where $X \indep_P Y$.

%It can be verified that the set of unfaithful observational distributions $P_{\model}$, with respect to $G(\model)=G$, is obtained by setting $p_1=1/2$. 

Given that observational data is generated from $\model \in \modelfamxor$, we now consider the question of testing whether the edge $X \rightarrow Y$ exists from samples drawn from $P_{\model}$. Specifically, we would like to test for the causal null hypothesis
\begin{equation}
    \nullcausalxor \triangleq \left \lbrace \model \in \modelfamxor: X  \rightarrow Y \notin G(\model) \right \rbrace.
\end{equation}
For the above causal null hypothesis, the set of observational distributions induced by $H^0_{\text{graph}}$ is simply the set of distributions on $X,Y$ such that $X$ and $Y$ are independent, i.e, 
\begin{equation}
    \distxor \triangleq \left \{ P_{\model} \in \Delta : \model \in \nullcausalxor \right \} = \left \{ P \in \Delta : X \indep_P Y \right \}.
\end{equation}
The implications of a binary-outcome independence test for $\nullcausalxor$ are similar to Section~\ref{sec:setup}, i.e., a binary-outcome independence test tests the causal null hypothesis 
\begin{equation*}
    \nullcausalxordist \triangleq \left \{ \model \in \modelfamxor : P_{\model} \in \distxor \right \} = \left \{ \model \in \modelfamxor :X \indep_{P_{\model}} Y \right \}.
\end{equation*}

Clearly, $\altnonidxor \triangleq \nullcausalxordist \cap \altcausalxor$ is the set of causal models that induce ``unfaithful'' distributions w.r.t. $G$ where the latter is defined as the set of distributions that are Markov w.r.t. $G$ and where $X \indep Y$. A concrete example for $\model \in \altnonidxor$ is given below
\begin{example}
Consider a subset of $\altcausalxor$, $\modelxor \triangleq \left \lbrace M \in \modelfamxor : f_Y(X,U_Y) = X \oplus U_Y \right \rbrace.$ Note that for every $\model \in \modelxor$, the causal graph, $G(\model) = G$. The set of observational distributions of $\modelxor $ are parameterized by $(p_0,p_1)$, and each element is represented as 
\begin{equation*}
    P_{\model}(x,y) = \begin{cases}
        (1-p_0)(1-p_1) &\text{ if } (x,y) = (0,0),\\
        (1-p_0)p_1 &\text{ if } (x,y) = (0,1),\\
        p_0p_1 &\text{ if } (x,y) = (1,0),\\
        p_0(1-p_1) &\text{ if } (x,y) = (1,1).\\
    \end{cases}
\end{equation*}
It can be verified that a subset of unfaithful observational distributions with respect to $G(\model)=G$, is obtained by setting $p_1=1/2$. 
\end{example}

The above example implies that a binary-outcome independence test that rejects the statistical null ($\distxor$) implies that a direct effect is present. However, not rejecting the statistical null does not imply that the direct effect is absent (ignoring finite-sample effects) since it is possible for $\model$ to have belonged to $\modelxor$ where $p_1=1/2$, i.e., it is possible that the data was drawn from an unfaithful distribution. Therefore, not rejecting the statistical null raises a ``identifiability'' issue and we should conclude that the absence of a direct effect, using a binary-outcome independence test, is ``unidentifiable''. 

For the considered query, $\distq = \left \{ P_{\model} \in \Delta: X \indep_{P_{\model}} Y \right \}$. However, without assuming faithfulness, $\distqalt  = \left \{ P_{\model} \in \Delta: \model \in \altcausalq \right \} = \Delta$ since it contains distributions that satisfy $X \not\indep_{P_{\model}} Y$ since $X \rightarrow Y \in G(\model)$ and it contains distributions that satisfy $X \indep_{P_{\model}} Y$ for unfaithful causal models in $\altcausalq$. Therefore, while the identifiability issue remains, an appropriate statistical test for this case suffices to be binary where if $X \not\indep Y$, then $\distq$ is rejected and in turn, so is $\nullcausalq$. Whereas if $X \indep Y$, then since $\distq = \distq \cap \distqalt$, the statistical test should output ``unidentifiable''.

The usual workaround to the issue that arises from unfaithful distributions is to assume that the distributions that we encounter are all faithful distributions.\todo{Add some comment on past results of typicality of faithful distributions that seemingly justify this assumption} This can be viewed as modifying $\modelfamxor$ to remove causal models that induce unfaithful distributions, i.e., to remove $\altnonidxor$ from $\modelfamxor$. Note that this is one of those cases where, by definition of the query and the problem setup, there is no $\model \in \nullcausalq$ such that $P_{\model} \in \distqalt$.

